Towards AI-Agent-Accelerated Research in High-Energy Physics: A Case Study in Monte Carlo Analysis

We investigate how far contemporary LLM-based agents can participate in multistep computational high-energy-physics research under reproducible human supervision. Using a previously published CEPC Bell-observable analysis in $e^+e^- \to ZH$, $Z \to q\bar q$, $H \to ZZ^* \to 4\mu$ as a case study, we test two capabilities. First, the agent performs an instruction-constrained reproduction: it is explicitly instructed not to use the published numerical results as analysis targets, although no technical information-access barrier is imposed. The analysis definition is fixed before the formal comparison, and the resulting detector-level $I_3$ central values reproduce the four published benchmark points to within about 2% without retuning to those values. Second, the agent is used for an open-ended extension with no target answer supplied. Using 200,000 fast-simulated events, a stage-resolved audit identifies muon isolation as the largest single contribution to the hard-to-detector shift, and subsequent diagnostics connect the effect to angle-dependent isolation efficiency, proximity to the hard $Z \to q\bar q$ system, and mixed electromagnetic activity from muon final-state radiation and hadron decays. Throughout, the agent assists with workflow planning, code and configuration inspection, Monte Carlo production, anomaly diagnosis, control construction, statistical analysis, and result organization, while state-changing actions and final interpretation remain under human control. The study shows that the value of AI agents in HEP may lie not only in faster code generation, but in faster scientific iteration, and motivates systematic benchmarking across historical HEP analyses using correctness, human intervention, and researcher-time efficiency as explicit metrics.

==> sections/03_simulation.tex <==
% \section{Simulation and event selection}
% \label{sec:simulation}

% \subsection{Event generation and showering}

% The signal process of Eq.~(1) is generated at $\sqrt{s}=250$~GeV, with the resonance decay chain encoded at matrix-element level.  The final production consists of 200 independent random seeds and 1000 events per seed, for a total of 200,000 events.  The original 20 seeds used in the earlier production are retained and 180 additional seeds extend the sample; no branching-fraction factor is applied after generation because the decay-chain branching fractions are already embedded in the generated process.

% The matrix-element samples were produced with MadGraph5\_aMC@NLO version~3.7.1~\cite{Alwall2014}.  Showering and hadronization use PYTHIA~8.317~\cite{Pythia83}.  The production steering has initial-state radiation disabled, QED final-state radiation and hadronization enabled, no pileup, and no beamstrahlung model.  Beam polarization is inherited from the LHE input and is zero for the production used here.  These choices are stated explicitly because they define the scope of the reproduction; no unreported beam-spectrum model is inferred from the earlier paper.

% The PYTHIA treatment of the massless LHE muons can shift dilepton masses by up to $\sim0.45$~GeV through recoil redistribution in a 1000-event control; this convention dependence is discussed in Appendix~\ref{app:controls}. The hard reference always uses the original LHE vectors.

% \subsection{Fast detector simulation}

% Detector response is simulated with Delphes~3.5.1~\cite{Delphes2014} using the CEPC detector card of Ref.~\cite{WuEtAl2025CEPC}, translated only where required for compatibility with the installed Delphes syntax.  No detector parameter is tuned to improve agreement in $I_3$.  The diagnostic configuration writes additional intermediate branches but leaves the physics modules and settings unchanged.

% For the muon chain, the CEPC card imposes the nominal energy/acceptance response with zero efficiency for $E<2$~GeV or $|\eta|>3$ and $99\%$ efficiency otherwise.  Muon isolation uses the pre-isolation candidates from the muon-efficiency module and particle-flow inputs from the filtered EFlow collection.  The isolation cone has $\Delta R=0.5$, includes constituents with $p_T\ge0.5$ GeV, and requires a relative scalar-$p_T$ sum not exceeding $0.25$.  The filtered isolation inputs remove identified electrons and muons; hence a signal muon does not directly contribute its own momentum to the isolation sum.  No $\rho$ input is supplied, so the corresponding correction is zero.  The reconstructed electron collection used by the electron veto follows the same nominal CEPC energy/acceptance response ($E>2$ GeV and $|\eta|<3$ in the active region).  Jets are clustered using FastJet~3.5.1~\cite{Cacciari2012FastJet}
% with the anti-$k_T$ algorithm~\cite{Cacciari2008AntiKt},
% using a radius parameter $R=0.5$ and a transverse-momentum
% threshold of 20~GeV.

% \subsection{Reconstruction and analysis selection}

% The stage audit follows the reconstructed object chain rather than collapsing it into a single detector selection.  The ordered stages are
% \begin{enumerate}[label=(\roman*)]
%  \item hard reference;
%  \item tracking geometry;
%  \item tracking smearing;
%  \item muon energy and pseudorapidity acceptance;
%  \item stochastic muon efficiency;
%  \item muon isolation;
%  \item overlap removal;
%  \item exactly four signal-matched reconstructed muons;
%  \item exactly two jets together with the electron veto;
%  \item opposite-sign pairing and the $Z_1$ mass window;
%  \item nominal detector-level kinematics and selection.
% \end{enumerate}
% The same-flavor pairing follows the convention of Ref.~\cite{WuEtAl2025CEPC}.  The larger dimuon mass is assigned to $Z_1$, the smaller to $Z_2$, and the strict on-shell window is
% \begin{equation}
%  \left|m_{Z_1}-91.1876~\mathrm{GeV}\right|<10~\mathrm{GeV}.
% \end{equation}
% The final ``nominal detector'' stage recomputes the dimuon pairing, rest-frame angles, and mass selections from the final reconstructed muon four-vectors; its event count can therefore differ slightly from the preceding frozen-mask stage through kinematic migrations.  Four nested $Z_2$ requirements are studied: $m_{Z_2}>0$, 10, 20, and 30 GeV.  Because these thresholds are nested, their statistical results are strongly correlated and are not interpreted as four independent confirmations.

% \figorplaceholder{event_yield_by_stage_clean.pdf}{Eligible event counts through the audited reconstruction and selection chain for the four nested $m_{Z_2}$ thresholds.  The final detector-level counts are 56,091, 51,575, 36,375, and 10,224.  The last stage contains migration effects and is shown as an event count rather than interpreted as a standalone efficiency.}{fig:eventflow}
\section{Simulation and frozen analysis selection}
\label{sec:simulation}

This section records the simulation and reconstruction specification that the agent was required to implement for the benchmark. The purpose is to make explicit which generator settings, detector definitions, and selection stages were fixed before the formal comparison with the published result and subsequently reused in the open-ended diagnostic study.

\subsection{Event generation and showering}

The reference process of Eq.~(1) is generated at $\sqrt{s}=250$~GeV, with the resonance decay chain encoded at matrix-element level. The final production consists of 200 random seeds and 1000 events per seed, for a total of 200,000 events. The original 20 development seeds are retained and 180 additional seeds enlarge the sample; no branching-fraction factor is applied after generation because the decay-chain branching fractions are already embedded in the generated process.

Matrix-element generation uses MadGraph5\_aMC@NLO version~3.7.1~\cite{Alwall2014}, followed by showering and hadronization with PYTHIA~8.317~\cite{Pythia83}. The frozen production steering has initial-state radiation disabled, QED final-state radiation and hadronization enabled, no pileup, and no beamstrahlung model. Beam polarization is inherited from the LHE input and is zero for the production used here. These settings are stated explicitly because part of the agentic task was to distinguish documented analysis choices from assumptions that were not specified in the reference material.

One development-stage control identified a convention dependence associated with PYTHIA's treatment of the massless LHE muons: recoil redistribution can shift dilepton masses by up to approximately $0.45$~GeV in a 1000-event control sample. This effect and the corresponding validation are discussed in Appendix~\ref{app:controls}. The frozen hard reference always uses the original LHE four-vectors.

\subsection{Fast detector simulation}

Detector response is simulated with Delphes~3.5.1~\cite{Delphes2014} using the CEPC detector card associated with Ref.~\cite{WuEtAl2025CEPC}. The card was translated only where required for compatibility with the installed Delphes syntax. This translation was treated as a software-compatibility intervention rather than as a physics retuning: same-seed validation was used to verify the response, and no detector parameter was adjusted to improve agreement in $I_3$. The diagnostic configuration writes additional intermediate branches while leaving the nominal physics modules and settings unchanged.

For the muon chain, the frozen detector definition has zero efficiency for $E<2$~GeV or $|\eta|>3$ and $99\%$ efficiency otherwise. Muon isolation operates on pre-isolation candidates from the muon-efficiency module and particle-flow inputs from the filtered EFlow collection. The isolation cone has $\Delta R=0.5$, includes constituents with $p_T\ge0.5$~GeV, and requires a relative scalar-$p_T$ sum not exceeding $0.25$. Identified electrons and muons are removed from the filtered isolation input, so a signal muon does not directly contribute its own momentum to the isolation sum. No $\rho$ input is supplied, and the corresponding correction is therefore zero.

The reconstructed electron collection used by the electron veto follows the same nominal CEPC energy and acceptance requirement, with $E>2$~GeV and $|\eta|<3$ in the active region. Jets are clustered using FastJet~3.5.1~\cite{Cacciari2012FastJet} with the anti-$k_T$ algorithm~\cite{Cacciari2008AntiKt}, a radius parameter $R=0.5$, and a transverse-momentum threshold of 20~GeV.

\subsection{Reconstruction and frozen analysis selection}

The frozen analysis specification records the reconstructed object chain stage by stage rather than collapsing detector reconstruction into a single selection. The ordered stages are
\begin{enumerate}[label=(\roman*)]
 \item hard reference;
 \item tracking geometry;
 \item tracking smearing;
 \item muon energy and pseudorapidity acceptance;
 \item stochastic muon efficiency;
 \item muon isolation;
 \item overlap removal;
 \item exactly four signal-matched reconstructed muons;
 \item exactly two jets together with the electron veto;
 \item opposite-sign pairing and the $Z_1$ mass window;
 \item nominal detector-level kinematics and selection.
\end{enumerate}

This ordering subsequently provides the basis for the stage-resolved agentic diagnosis. The same-flavor pairing follows Ref.~\cite{WuEtAl2025CEPC}: the larger dimuon mass is assigned to $Z_1$ and the smaller to $Z_2$. The strict on-shell requirement is
\begin{equation}
 \left|m_{Z_1}-91.1876~\mathrm{GeV}\right|<10~\mathrm{GeV}.
\end{equation}
The final ``nominal detector'' stage recomputes the dimuon pairing, rest-frame angles, and mass selections from the final reconstructed muon four-vectors; its event count can therefore differ slightly from the preceding frozen-mask stage through kinematic migration.

Four nested $Z_2$ requirements are evaluated:
\[
m_{Z_2}>0,\ 10,\ 20,\ 30~\mathrm{GeV}.
\]
Because these selections are nested, their statistical results are strongly correlated and are not interpreted as four independent confirmations.

\figorplaceholder{event_yield_by_stage_clean.pdf}{
Eligible event counts through the frozen reconstruction and selection chain for the four nested $m_{Z_2}$ thresholds. The final detector-level counts are 56,091, 51,575, 36,375, and 10,224. The final stage includes kinematic-migration effects and is shown as an event count rather than interpreted as a standalone efficiency.
}{fig:eventflow}

These settings define the frozen technical task used in the instruction-constrained benchmark. The next section describes how the agentic workflow executed this specification and compares the resulting observable with the published CEPC values only after the analysis configuration had been fixed.
